Deep Reinforcement Learning for Haptic Shared Control in Unknown Tasks

Recent years have shown a growing interest in using haptic shared control (HSC) in teleoperated systems. In HSC, the application of virtual guiding forces decreases the user's control effort and improves execution time in various tasks, presenting a good alternative in comparison with direct teleoperation. HSC, despite demonstrating good performance, opens a new gap: how to design the guiding forces. For this reason, the challenge lies in developing controllers to provide the optimal guiding forces for the tasks that are being performed. This work addresses this challenge by designing a controller based on the deep deterministic policy gradient (DDPG) algorithm to provide the assistance, and a convolutional neural network (CNN) to perform the task detection, called TAHSC (Task Agnostic Haptic Shared Controller). The agent learns to minimize the time it takes the human to execute the desired task, while simultaneously minimizing their resistance to the provided feedback. This resistance thus provides the learning algorithm with information about which direction the human is trying to follow, in this case, the pick-and-place task. Diverse results demonstrate the successful application of the proposed approach by learning custom policies for each user who was asked to test the system. It exhibits stable convergence and aids the user in completing the task with the least amount of time possible.

==> algorithms/section_4/Teleoperation.tex <==
\begin{algorithmic}
\Function{Teleoperation-controller}{\null}
    % \State $\touchPosF \leftarrow 0, \dobotPosF \leftarrow 0$
    \While{True}
        \State Read $\touchPosF$, $\dobotPosF$
        \State $\xF{Dd} \leftarrow -\xF{T}$
        \State $\yF{Dd} \leftarrow 1.4 \zF{T} + 0.2464$
        \State $\zF{Dd} \leftarrow \yF{T} + 0.098$
        \State $\dobotPosFd \leftarrow \cVectorF{Dd}$
        \State $\vectorF{e} = \dobotPosFd - \dobotPosF$
        \State $\dobotVelVF = k_D \vectorF{e}$
        \State Send $\dobotVelVF$ to Dobot
    \EndWhile
\EndFunction
\end{algorithmic}

==> algorithms/section_5/DDPGsimulator.tex <==
\begin{algorithmic}
\Function{DDPG}{$\discountF, \tau, M, N$}%{$\tau$}
\State Initialize $\criticPVF, \actorPVF, \targetCriticPVF, \targetActorPVF$ with random values close to zero
\State $n \leftarrow 0$, $t \leftarrow 0$, $\mathit{task} \leftarrow 0$
%\State $M \leftarrow 2\mathrm{epochs}$
%\State $N \leftarrow \mathrm{batch\ size}$
\For{episode=1,M}
    % \State Set $\mathit{execution} \leftarrow 1$
    \State $\sF \leftarrow$ Start for \textit{task}
    \While{$\sF\ \mathrm{is}\ \mathbf{not}\ \sF_{n}$}
        \State Select action $\actionF$ from $\detParamPolFtime + \arpProcess_t$
        \State Execute action $\actionF$, observe reward $\rF$ and observe new state $\sF'_{t}$
        \State Store transition $(\sF_{t},\aF_{t},\rF_{t},\sF'_{t}, 0)$ in $\bufferF$
        \State $\sF_t \leftarrow \nSF_t$
        \State $n \leftarrow n+1$
        \State $t \leftarrow t+1$
        % \If{$\sF = \finalStateF$}
        %     \State Set $\mathit{execution} \leftarrow 0$
        % \EndIf
    \EndWhile
    \State $\rF_n \leftarrow \rF_n+10$
    \State Store transition $(\sF_{n},\aF_{n},\rF_{n},\sF'_{n}, 1)$ in $\bufferF$
    \For{steps=1,n}
        \State \Call{Train-minibatch}{$\bufferF, \discountF, \tau, \actorPVF, \targetActorPVF, \criticPVF, \targetCriticPVF, N$}
        % \State $\sF \leftarrow \nSF$
    \EndFor
    \State $\mathit{task} \leftarrow \mathbf{not}\ \mathit{task}$
\EndFor
\EndFunction
% \Statex
% \Function{Train-minibatch}{$\batchF, \discountF, \tau, \actorPVF, \targetActorPVF, \criticPVF, \targetCriticPVF$}
%     \State Sample a random minibatch $\batchF \subset \bufferF$ of size $N$
%     \For{each $b_i: (\sF_i,\aF_i,\rF_i,\nSF_i) \in \batchF$}
%         \State $y_{i} = \rF_{i} + \gamma \ndetParamQF$
%     \EndFor
%     \State Train $\detParamAppQF$ on all samples $N$
%     \State Move $\detParamPolF$ according to the sampled deterministic policy gradient 
%     \State $\frac{1}{N} \sumaF{1}{N} [\grad_{a} \detParamQF \vert_{s=s_i,a=\idetParamPolF} \grad_{\actorPVF} \detParamPolF \vert_{s=s_i}]$
%     \State $\targetActorPVF \leftarrow \targetActorPVF + \tau (\actorPVF - \targetActorPVF)$
%     \State $\targetCriticPVF \leftarrow \targetCriticPVF + \tau (\criticPVF - \targetCriticPVF)$
% \EndFunction
\Statex
\Function{Train-minibatch}{$\bufferF, \discountF, \tau, \actorPVF, \targetActorPVF, \criticPVF, \targetCriticPVF, N$}
    \State Sample a random minibatch $\batchF \subset \bufferF$ of size $N$
    \For{each $b_i: (\sF_i,\aF_i,\rF_i,\nSF_i, \mathrm{A}_i) \in \batchF$}
        \If{$\mathrm{A}_i = 0$}
            \State $y_{i} = \rF_{i} + \gamma \indetParamQF$
        \Else
            \State $y_{i} = \rF_{i} $
        \EndIf
        
    \EndFor
    \State Train $\detParamAppQF$ on all samples $N$
    \State Move $\detParamPolF$ according to the sampled deterministic policy gradient 
    \State $\frac{1}{N} \sumaF{1}{N} [\grad_{\aF} \detParamQF \vert_{\sF=\sF_i,\aF=\idetParamPolF} \grad_{\actorPVF} \detParamPolF \vert_{\sF=\sF_i}]$
    \State $\targetActorPVF \leftarrow \targetActorPVF + \tau (\actorPVF - \targetActorPVF)$
    \State $\targetCriticPVF \leftarrow \targetCriticPVF + \tau (\criticPVF - \targetCriticPVF)$
\EndFunction
\end{algorithmic}


==> figures/introduction/systemOverview.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,703); %set diagram left start at 0, and has height of 703

%Rounded Rect [id:dp2760368533505071] 
\draw   (70,84) .. controls (70,79.58) and (73.58,76) .. (78,76) -- (103,76) .. controls (107.42,76) and (111,79.58) .. (111,84) -- (111,108) .. controls (111,112.42) and (107.42,116) .. (103,116) -- (78,116) .. controls (73.58,116) and (70,112.42) .. (70,108) -- cycle ;
%Rounded Rect [id:dp1417896057221032] 
\draw   (150,84) .. controls (150,79.58) and (153.58,76) .. (158,76) -- (201,76) .. controls (205.42,76) and (209,79.58) .. (209,84) -- (209,108) .. controls (209,112.42) and (205.42,116) .. (201,116) -- (158,116) .. controls (153.58,116) and (150,112.42) .. (150,108) -- cycle ;
%Rounded Rect [id:dp8320759149216168] 
\draw   (247,84) .. controls (247,79.58) and (250.58,76) .. (255,76) -- (309,76) .. controls (313.42,76) and (317,79.58) .. (317,84) -- (317,108) .. controls (317,112.42) and (313.42,116) .. (309,116) -- (255,116) .. controls (250.58,116) and (247,112.42) .. (247,108) -- cycle ;
%Rounded Rect [id:dp01188410540048146] 
\draw   (355,84) .. controls (355,79.58) and (358.58,76) .. (363,76) -- (407,76) .. controls (411.42,76) and (415,79.58) .. (415,84) -- (415,108) .. controls (415,112.42) and (411.42,116) .. (407,116) -- (363,116) .. controls (358.58,116) and (355,112.42) .. (355,108) -- cycle ;
%Rounded Rect [id:dp4645214777815967] 
\draw   (355,140) .. controls (355,137.24) and (357.24,135) .. (360,135) -- (410,135) .. controls (412.76,135) and (415,137.24) .. (415,140) -- (415,155) .. controls (415,157.76) and (412.76,160) .. (410,160) -- (360,160) .. controls (357.24,160) and (355,157.76) .. (355,155) -- cycle ;
%Straight Lines [id:da3313679184976388] 
\draw    (355,145) -- (280,145) -- (280,118) ;
\draw [shift={(280,115)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da4543348029914457] 
\draw    (111,108) -- (147,108) ;
\draw [shift={(150,108)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da40879237109204114] 
\draw    (150,84) -- (114,84) ;
\draw [shift={(111,84)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da2555337367701145] 
\draw    (209,108) -- (244,108) ;
\draw [shift={(247,108)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da7958142793147414] 
\draw    (317,108) -- (352,108) ;
\draw [shift={(355,108)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da8131129993324346] 
\draw    (247,84) -- (212,84) ;
\draw [shift={(209,84)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da0016306205044754885] 
\draw    (355,84) -- (320,84) ;
\draw [shift={(317,84)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da9907578347576678] 
\draw    (385,132) -- (385,116) ;
\draw [shift={(385,135)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Rectangle [id:dp37498627380741545] 
\draw  [dash pattern={on 4.5pt off 4.5pt}] (60,30) -- (225,30) -- (225,151) -- (60,151) -- cycle ;
%Shape: Rectangle [id:dp5296722097463731] 
\draw  [dash pattern={on 4.5pt off 4.5pt}] (340,30) -- (425,30) -- (425,185) -- (340,185) -- cycle ;

% Text Node
\draw (385.5,54) node   [align=left] {\begin{minipage}[lt]{34.838644pt}\setlength\topsep{0pt}
\begin{center}
SLAVE\\SIDE
\end{center}

\end{minipage}};
% Text Node
\draw (143,54.5) node   [align=left] {MASTER SIDE};
% Text Node
\draw (385,147.5) node   [align=left] {Camera};
% Text Node
\draw (385,96) node   [align=left] {\begin{minipage}[lt]{37.320644pt}\setlength\topsep{0pt}
\begin{center}
Robotic\\arm
\end{center}

\end{minipage}};
% Text Node
\draw (282,96) node   [align=left] {Controller};
% Text Node
\draw (179.5,96) node   [align=left] {\begin{minipage}[lt]{32.220644pt}\setlength\topsep{0pt}
\begin{center}
Haptic\\device
\end{center}

\end{minipage}};
% Text Node
\draw (90.5,96) node   [align=left] {User};


\end{tikzpicture}


==> figures/section_2/flowchart.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,703); %set diagram left start at 0, and has height of 703

%Straight Lines [id:da7771436051327765] 
\draw    (130,403) -- (167,403) ;
\draw [shift={(170,403)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da9635197088307833] 
\draw    (170,379) -- (133,379) ;
\draw [shift={(130,379)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da12330573086743057] 
\draw    (285,380) -- (233,380) ;
\draw [shift={(230,380)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Rounded Rect [id:dp7108259694514127] 
\draw   (265,329.7) .. controls (265,324.34) and (269.34,320) .. (274.7,320) -- (390.3,320) .. controls (395.66,320) and (400,324.34) .. (400,329.7) -- (400,480.3) .. controls (400,485.66) and (395.66,490) .. (390.3,490) -- (274.7,490) .. controls (269.34,490) and (265,485.66) .. (265,480.3) -- cycle ;
%Rounded Rect [id:dp1931664995958754] 
\draw   (445,382) .. controls (445,378.13) and (448.13,375) .. (452,375) -- (516,375) .. controls (519.87,375) and (523,378.13) .. (523,382) -- (523,403) .. controls (523,406.87) and (519.87,410) .. (516,410) -- (452,410) .. controls (448.13,410) and (445,406.87) .. (445,403) -- cycle ;
%Shape: Rectangle [id:dp38727394979643515] 
\draw  [dash pattern={on 4.5pt off 4.5pt}] (429,320) -- (535,320) -- (535,490) -- (429,490) -- cycle ;
%Rounded Rect [id:dp012625308412551606] 
\draw   (449,336) .. controls (449,332.69) and (451.69,330) .. (455,330) -- (513,330) .. controls (516.31,330) and (519,332.69) .. (519,336) -- (519,354) .. controls (519,357.31) and (516.31,360) .. (513,360) -- (455,360) .. controls (451.69,360) and (449,357.31) .. (449,354) -- cycle ;
%Straight Lines [id:da5298843006880326] 
\draw    (485,375) -- (485,363) ;
\draw [shift={(485,360)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da07336353433707032] 
\draw    (229,405.5) -- (275,405) -- (275,440) -- (282,440) ;
\draw [shift={(285,440)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (6.25,-3) -- (0,0) -- (6.25,3) -- cycle    ;
%Straight Lines [id:da12778070597856206] 
\draw    (275,405) -- (330,405) -- (330,398) ;
\draw [shift={(330,395)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (6.25,-3) -- (0,0) -- (6.25,3) -- cycle    ;
%Straight Lines [id:da8660777208935828] 
\draw    (380,450) -- (405,450) -- (405,400) -- (442,400) ;
\draw [shift={(445,400)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da4968165023134957] 
\draw    (445,380) -- (383,380) ;
\draw [shift={(380,380)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da13650811678684382] 
\draw    (450,350) -- (330,350) -- (330,362) ;
\draw [shift={(330,365)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (6.25,-3) -- (0,0) -- (6.25,3) -- cycle    ;
%Straight Lines [id:da49568575505555357] 
\draw    (395,380) -- (395,425) -- (383,425) ;
\draw [shift={(380,425)}, rotate = 360] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Flowchart: Connector [id:dp19483205865008557] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (272.5,405) .. controls (272.5,403.62) and (273.62,402.5) .. (275,402.5) .. controls (276.38,402.5) and (277.5,403.62) .. (277.5,405) .. controls (277.5,406.38) and (276.38,407.5) .. (275,407.5) .. controls (273.62,407.5) and (272.5,406.38) .. (272.5,405) -- cycle ;
%Flowchart: Connector [id:dp22889773082518394] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (392.5,380) .. controls (392.5,378.62) and (393.62,377.5) .. (395,377.5) .. controls (396.38,377.5) and (397.5,378.62) .. (397.5,380) .. controls (397.5,381.38) and (396.38,382.5) .. (395,382.5) .. controls (393.62,382.5) and (392.5,381.38) .. (392.5,380) -- cycle ;
%Rounded Rect [id:dp9131901255796766] 
\draw   (285,371) .. controls (285,367.69) and (287.69,365) .. (291,365) -- (374,365) .. controls (377.31,365) and (380,367.69) .. (380,371) -- (380,389) .. controls (380,392.31) and (377.31,395) .. (374,395) -- (291,395) .. controls (287.69,395) and (285,392.31) .. (285,389) -- cycle ;
%Rounded Rect [id:dp48963258471872295] 
\draw   (89,379) .. controls (89,374.58) and (92.58,371) .. (97,371) -- (122,371) .. controls (126.42,371) and (130,374.58) .. (130,379) -- (130,403) .. controls (130,407.42) and (126.42,411) .. (122,411) -- (97,411) .. controls (92.58,411) and (89,407.42) .. (89,403) -- cycle ;
%Rounded Rect [id:dp16854676256906764] 
\draw   (170,379) .. controls (170,374.58) and (173.58,371) .. (178,371) -- (221,371) .. controls (225.42,371) and (229,374.58) .. (229,379) -- (229,403) .. controls (229,407.42) and (225.42,411) .. (221,411) -- (178,411) .. controls (173.58,411) and (170,407.42) .. (170,403) -- cycle ;
%Shape: Rectangle [id:dp16721018575840352] 
\draw  [dash pattern={on 4.5pt off 4.5pt}] (75,339) -- (240,339) -- (240,460) -- (75,460) -- cycle ;
%Rounded Rect [id:dp9522356594280785] 
\draw   (285,424) .. controls (285,419.03) and (289.03,415) .. (294,415) -- (371,415) .. controls (375.97,415) and (380,419.03) .. (380,424) -- (380,451) .. controls (380,455.97) and (375.97,460) .. (371,460) -- (294,460) .. controls (289.03,460) and (285,455.97) .. (285,451) -- cycle ;

% Text Node
\draw (484.5,456) node   [align=left] {\begin{minipage}[lt]{34.838644pt}\setlength\topsep{0pt}
\begin{center}
SLAVE\\SIDE
\end{center}

\end{minipage}};
% Text Node
\draw (484,392.5) node  [font=\small] [align=left] {\begin{minipage}[lt]{50.660000000000004pt}\setlength\topsep{0pt}
\begin{center}
Robotic\\manipulator
\end{center}

\end{minipage}};
% Text Node
\draw (157,445.5) node   [align=left] {MASTER SIDE};
% Text Node
\draw (147,410) node    {$\boldsymbol{p}$};
% Text Node
\draw (254.5,414) node    {$\boldsymbol{p}_{\mathrm{T}}$};
% Text Node
\draw (254,369) node    {$\boldsymbol{f}_{\mathrm{T}}$};
% Text Node
\draw (151,364) node    {$\boldsymbol{f}$};
% Text Node
\draw (376,340) node    {$task$};
% Text Node
\draw (416.5,369) node    {$\boldsymbol{p}_{\mathrm{D}}$};
% Text Node
\draw (418.5,413) node    {$\dot{\boldsymbol{p}}_{\mathrm{D}}$};
% Text Node
\draw (331.5,475.5) node   [align=left] {CONTROLLER};
% Text Node
\draw (484,345) node   [align=left] {Camera};
% Text Node
\draw (332.5,437.5) node   [align=left] {\begin{minipage}[lt]{64.01064400000001pt}\setlength\topsep{0pt}
\begin{center}
Teleoperation\\controller
\end{center}

\end{minipage}};
% Text Node
\draw (332.5,380) node   [align=left] {RL-controller};
% Text Node
\draw (109.5,391) node   [align=left] {User};
% Text Node
\draw (199.5,391) node   [align=left] {\begin{minipage}[lt]{32.220644pt}\setlength\topsep{0pt}
\begin{center}
Haptic\\device
\end{center}

\end{minipage}};


\end{tikzpicture}


==> figures/section_2/flowchartRLcontroller.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,3250); %set diagram left start at 0, and has height of 3250

%Rounded Rect [id:dp5127697938256253] 
\draw   (225,953.23) .. controls (225,951.45) and (226.45,950) .. (228.23,950) -- (306.77,950) .. controls (308.55,950) and (310,951.45) .. (310,953.23) -- (310,991.77) .. controls (310,993.55) and (308.55,995) .. (306.77,995) -- (228.23,995) .. controls (226.45,995) and (225,993.55) .. (225,991.77) -- cycle ;
%Rounded Rect [id:dp990066090666564] 
\draw   (330,953.23) .. controls (330,951.45) and (331.45,950) .. (333.23,950) -- (471.77,950) .. controls (473.55,950) and (475,951.45) .. (475,953.23) -- (475,991.77) .. controls (475,993.55) and (473.55,995) .. (471.77,995) -- (333.23,995) .. controls (331.45,995) and (330,993.55) .. (330,991.77) -- cycle ;
%Rounded Rect [id:dp41517782253315816] 
\draw   (480,868.23) .. controls (480,866.45) and (481.45,865) .. (483.23,865) -- (576.77,865) .. controls (578.55,865) and (580,866.45) .. (580,868.23) -- (580,906.77) .. controls (580,908.55) and (578.55,910) .. (576.77,910) -- (483.23,910) .. controls (481.45,910) and (480,908.55) .. (480,906.77) -- cycle ;
%Rounded Rect [id:dp7200651652350234] 
\draw   (220,1173.23) .. controls (220,1171.45) and (221.45,1170) .. (223.23,1170) -- (316.77,1170) .. controls (318.55,1170) and (320,1171.45) .. (320,1173.23) -- (320,1211.77) .. controls (320,1213.55) and (318.55,1215) .. (316.77,1215) -- (223.23,1215) .. controls (221.45,1215) and (220,1213.55) .. (220,1211.77) -- cycle ;
%Rounded Rect [id:dp8002540604399623] 
\draw   (215,1018.23) .. controls (215,1016.45) and (216.45,1015) .. (218.23,1015) -- (321.77,1015) .. controls (323.55,1015) and (325,1016.45) .. (325,1018.23) -- (325,1056.77) .. controls (325,1058.55) and (323.55,1060) .. (321.77,1060) -- (218.23,1060) .. controls (216.45,1060) and (215,1058.55) .. (215,1056.77) -- cycle ;
%Rounded Rect [id:dp060927409062295435] 
\draw   (490,803.23) .. controls (490,801.45) and (491.45,800) .. (493.23,800) -- (566.77,800) .. controls (568.55,800) and (570,801.45) .. (570,803.23) -- (570,841.77) .. controls (570,843.55) and (568.55,845) .. (566.77,845) -- (493.23,845) .. controls (491.45,845) and (490,843.55) .. (490,841.77) -- cycle ;
%Straight Lines [id:da7650634976810728] 
\draw    (530,865) -- (530,848) ;
\draw [shift={(530,845)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Rounded Rect [id:dp5567448150471792] 
\draw   (85,808.23) .. controls (85,806.45) and (86.45,805) .. (88.23,805) -- (196.77,805) .. controls (198.55,805) and (200,806.45) .. (200,808.23) -- (200,846.77) .. controls (200,848.55) and (198.55,850) .. (196.77,850) -- (88.23,850) .. controls (86.45,850) and (85,848.55) .. (85,846.77) -- cycle ;
%Rounded Rect [id:dp2210530705908874] 
\draw   (80,868.59) .. controls (80,866.61) and (81.61,865) .. (83.59,865) -- (201.41,865) .. controls (203.39,865) and (205,866.61) .. (205,868.59) -- (205,911.41) .. controls (205,913.39) and (203.39,915) .. (201.41,915) -- (83.59,915) .. controls (81.61,915) and (80,913.39) .. (80,911.41) -- cycle ;
%Straight Lines [id:da013059274568433699] 
\draw    (140,850) -- (140,862) ;
\draw [shift={(140,865)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Rounded Rect [id:dp7861574401371162] 
\draw   (80,958.59) .. controls (80,956.61) and (81.61,955) .. (83.59,955) -- (201.41,955) .. controls (203.39,955) and (205,956.61) .. (205,958.59) -- (205,1001.41) .. controls (205,1003.39) and (203.39,1005) .. (201.41,1005) -- (83.59,1005) .. controls (81.61,1005) and (80,1003.39) .. (80,1001.41) -- cycle ;
%Rounded Rect [id:dp4429942193676458] 
\draw   (80,1088.23) .. controls (80,1086.45) and (81.45,1085) .. (83.23,1085) -- (201.77,1085) .. controls (203.55,1085) and (205,1086.45) .. (205,1088.23) -- (205,1126.77) .. controls (205,1128.55) and (203.55,1130) .. (201.77,1130) -- (83.23,1130) .. controls (81.45,1130) and (80,1128.55) .. (80,1126.77) -- cycle ;
%Rounded Rect [id:dp5319751205574779] 
\draw   (495,953.23) .. controls (495,951.45) and (496.45,950) .. (498.23,950) -- (566.77,950) .. controls (568.55,950) and (570,951.45) .. (570,953.23) -- (570,991.77) .. controls (570,993.55) and (568.55,995) .. (566.77,995) -- (498.23,995) .. controls (496.45,995) and (495,993.55) .. (495,991.77) -- cycle ;
%Straight Lines [id:da35569536315377503] 
\draw    (140,915) -- (140,952) ;
\draw [shift={(140,955)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da8245642574745367] 
\draw    (140,1085) -- (140,1008) ;
\draw [shift={(140,1005)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da5102914871915899] 
\draw    (205,975) -- (222,975) ;
\draw [shift={(225,975)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da09997615297815021] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (33,1068.5) -- (630,1068.5)(33,1071.5) -- (630,1071.5) ;
%Straight Lines [id:da267429491181821] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (33,923.5) -- (630,923.5)(33,926.5) -- (630,926.5) ;
%Straight Lines [id:da9370040737505719] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (33,1158.5) -- (630,1158.5)(33,1161.5) -- (630,1161.5) ;
%Straight Lines [id:da6289546366428818] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (33,794.17) -- (632,794.17)(33,797.17) -- (632,797.17) ;
%Straight Lines [id:da5888045112697865] 
\draw    (310,975) -- (327,975) ;
\draw [shift={(330,975)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da09963442904526232] 
\draw    (475,975) -- (492,975) ;
\draw [shift={(495,975)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da5856422260415305] 
\draw    (270,1015) -- (270,998) ;
\draw [shift={(270,995)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da8890107402294929] 
\draw    (530,950) -- (530,913) ;
\draw [shift={(530,910)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da993974979071755] 
\draw    (270,1170) -- (270,1063) ;
\draw [shift={(270,1060)}, rotate = 450] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da3171935661019387] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (33,1223.5) -- (630,1223.5)(33,1226.5) -- (630,1226.5) ;

% Text Node
\draw (530,822.5) node  [font=\large] [align=left] {\begin{minipage}[lt]{66.005356pt}\setlength\topsep{0pt}
\begin{center}
Assist user \\movements
\end{center}

\end{minipage}};
% Text Node
\draw (270,1037.5) node  [font=\large] [align=left] {\begin{minipage}[lt]{89.828pt}\setlength\topsep{0pt}
\begin{center}
Receive images\\from camera
\end{center}

\end{minipage}};
% Text Node
\draw (270,1192.5) node  [font=\large] [align=left] {\begin{minipage}[lt]{72.13644000000001pt}\setlength\topsep{0pt}
\begin{center}
Capture task\\images
\end{center}

\end{minipage}};
% Text Node
\draw (530,887.5) node  [font=\large] [align=left] {\begin{minipage}[lt]{83.69644000000001pt}\setlength\topsep{0pt}
\begin{center}
Execute forces\\commands
\end{center}

\end{minipage}};
% Text Node
\draw (402.5,972.5) node  [font=\large] [align=left] {\begin{minipage}[lt]{109.52556000000001pt}\setlength\topsep{0pt}
\begin{center}
Process inputs\\with DDPG network
\end{center}

\end{minipage}};
% Text Node
\draw (267.5,972.5) node  [font=\large] [align=left] {\begin{minipage}[lt]{64.645356pt}\setlength\topsep{0pt}
\begin{center}
Preprocess\\inputs
\end{center}

\end{minipage}};
% Text Node
\draw (55.5,858) node  [font=\large,rotate=-270] [align=left] {Haptic device};
% Text Node
\draw (56,1116) node  [font=\large,rotate=-270] [align=left] {\begin{minipage}[lt]{66.708pt}\setlength\topsep{0pt}
\begin{center}
Robotic\\manipulator
\end{center}

\end{minipage}};
% Text Node
\draw (54.5,990) node  [font=\large,rotate=-270] [align=left] {\begin{minipage}[lt]{72.81644pt}\setlength\topsep{0pt}
\begin{center}
RL-controller
\end{center}

\end{minipage}};
% Text Node
\draw (532.5,972.5) node  [font=\large] [align=left] {\begin{minipage}[lt]{62.605356pt}\setlength\topsep{0pt}
\begin{center}
Send force\\commands
\end{center}

\end{minipage}};
% Text Node
\draw (142.5,977.5) node  [font=\large] [align=left] {\begin{minipage}[lt]{99.35956pt}\setlength\topsep{0pt}
\begin{center}
Read tip position\\from both devices
\end{center}

\end{minipage}};
% Text Node
\draw (142.5,827.5) node  [font=\large] [align=left] {\begin{minipage}[lt]{74.868pt}\setlength\topsep{0pt}
\begin{center}
Encode user \\movements
\end{center}

\end{minipage}};
% Text Node
\draw (142.5,1107.5) node  [font=\large] [align=left] {\begin{minipage}[lt]{93.25044000000001pt}\setlength\topsep{0pt}
\begin{center}
Send tip position\\to controller
\end{center}

\end{minipage}};
% Text Node
\draw (142.5,890) node  [font=\large] [align=left] {\begin{minipage}[lt]{93.25044000000001pt}\setlength\topsep{0pt}
\begin{center}
Send tip position\\to controller
\end{center}

\end{minipage}};
% Text Node
\draw (59.5,1191.5) node  [font=\large,rotate=-270] [align=left] {Camera};


\end{tikzpicture}


==> figures/section_2/left.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,1903); %set diagram left start at 0, and has height of 1903

%Shape: Circle [id:dp588879061821758] 
\draw  [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][fill={rgb, 255:red, 244; green, 149; blue, 49 }  ,fill opacity=1 ] (481.83,1427.33) .. controls (481.83,1413.53) and (493.03,1402.33) .. (506.83,1402.33) .. controls (520.64,1402.33) and (531.83,1413.53) .. (531.83,1427.33) .. controls (531.83,1441.14) and (520.64,1452.33) .. (506.83,1452.33) .. controls (493.03,1452.33) and (481.83,1441.14) .. (481.83,1427.33) -- cycle ;
%Curve Lines [id:da06348859043456323] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=2.25]  [dash pattern={on 2.53pt off 3.02pt}]  (509.9,1436.01) .. controls (553.96,1446.21) and (571.4,1481.23) .. (568.5,1515) ;
\draw [shift={(505,1435)}, rotate = 10.3] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;
%Shape: Can [id:dp5283619466431455] 
\draw   (468.17,1496.38) -- (503.29,1461.26) .. controls (512.99,1451.56) and (528.74,1451.59) .. (538.48,1461.32) .. controls (548.21,1471.05) and (548.24,1486.81) .. (538.54,1496.5) -- (503.42,1531.63) .. controls (493.72,1541.32) and (477.97,1541.3) .. (468.23,1531.56) .. controls (458.5,1521.83) and (458.47,1506.08) .. (468.17,1496.38) .. controls (477.87,1486.68) and (493.62,1486.71) .. (503.36,1496.44) .. controls (513.09,1506.17) and (513.12,1521.93) .. (503.42,1531.63) ;
%Straight Lines [id:da8989387075173478] 
\draw    (384,1549) -- (642,1549) ;
%Shape: Ellipse [id:dp11328914028834136] 
\draw   (395,1521) .. controls (395,1517.13) and (403.28,1514) .. (413.5,1514) .. controls (423.72,1514) and (432,1517.13) .. (432,1521) .. controls (432,1524.87) and (423.72,1528) .. (413.5,1528) .. controls (403.28,1528) and (395,1524.87) .. (395,1521) -- cycle ;
%Shape: Ellipse [id:dp513276443206012] 
\draw   (550,1522) .. controls (550,1518.13) and (558.28,1515) .. (568.5,1515) .. controls (578.72,1515) and (587,1518.13) .. (587,1522) .. controls (587,1525.87) and (578.72,1529) .. (568.5,1529) .. controls (558.28,1529) and (550,1525.87) .. (550,1522) -- cycle ;
%Rounded Rect [id:dp9429679884563592] 
\draw   (503.79,1381.27) .. controls (503.79,1380.64) and (504.3,1380.13) .. (504.93,1380.13) -- (508.33,1380.13) .. controls (508.96,1380.13) and (509.47,1380.64) .. (509.47,1381.27) -- (509.47,1399.4) .. controls (509.47,1400.02) and (508.96,1400.53) .. (508.33,1400.53) -- (504.93,1400.53) .. controls (504.3,1400.53) and (503.79,1400.02) .. (503.79,1399.4) -- cycle ;
%Rounded Rect [id:dp4538921485752141] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (498.53,1373.05) .. controls (498.53,1371.33) and (499.93,1369.93) .. (501.65,1369.93) -- (511.01,1369.93) .. controls (512.74,1369.93) and (514.13,1371.33) .. (514.13,1373.05) -- (514.13,1387.21) .. controls (514.13,1388.94) and (512.74,1390.33) .. (511.01,1390.33) -- (501.65,1390.33) .. controls (499.93,1390.33) and (498.53,1388.94) .. (498.53,1387.21) -- cycle ;
%Shape: Cube [id:dp8145600773275845] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (489.83,1331.54) -- (510.04,1311.33) -- (539.33,1311.33) -- (539.33,1357.13) -- (519.13,1377.33) -- (489.83,1377.33) -- cycle ; \draw   (539.33,1311.33) -- (519.13,1331.54) -- (489.83,1331.54) ; \draw   (519.13,1331.54) -- (519.13,1377.33) ;
%Shape: Cube [id:dp6572864457379441] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (496.63,1298.83) -- (504.13,1291.33) -- (532.83,1291.33) -- (532.83,1318.04) -- (525.34,1325.54) -- (496.63,1325.54) -- cycle ; \draw   (532.83,1291.33) -- (525.34,1298.83) -- (496.63,1298.83) ; \draw   (525.34,1298.83) -- (525.34,1325.54) ;
%Rounded Rect [id:dp47880406996191105] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (508.73,1325.23) .. controls (508.73,1324.74) and (509.14,1324.33) .. (509.63,1324.33) -- (515.83,1324.33) .. controls (516.33,1324.33) and (516.73,1324.74) .. (516.73,1325.23) -- (516.73,1327.93) .. controls (516.73,1328.43) and (516.33,1328.83) .. (515.83,1328.83) -- (509.63,1328.83) .. controls (509.14,1328.83) and (508.73,1328.43) .. (508.73,1327.93) -- cycle ;
%Rounded Rect [id:dp6050305300120458] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (497.73,1325.23) .. controls (497.73,1324.74) and (498.14,1324.33) .. (498.63,1324.33) -- (504.83,1324.33) .. controls (505.33,1324.33) and (505.73,1324.74) .. (505.73,1325.23) -- (505.73,1327.93) .. controls (505.73,1328.43) and (505.33,1328.83) .. (504.83,1328.83) -- (498.63,1328.83) .. controls (498.14,1328.83) and (497.73,1328.43) .. (497.73,1327.93) -- cycle ;
%Shape: Diagonal Stripe [id:dp7729132516368667] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (514.43,1399.73) -- (521.83,1407.13) -- (492.23,1407.13) -- (499.63,1399.73) -- cycle ;

% Text Node
\draw (515.5,1479.5) node  [font=\large] [align=left] {Obstacle};
% Text Node
\draw (587,1349) node  [font=\normalsize] [align=left] {\begin{minipage}[lt]{67.852644pt}\setlength\topsep{0pt}
\begin{center}
{\large Manipulator}\\{\large end-effector}
\end{center}

\end{minipage}};
% Text Node
\draw (570,1537.5) node  [font=\large] [align=left] {Initial point};
% Text Node
\draw (414,1537.5) node  [font=\large] [align=left] {Goal};


\end{tikzpicture}


==> figures/section_2/right.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,1903); %set diagram left start at 0, and has height of 1903

%Shape: Can [id:dp4949158249688743] 
\draw   (146.17,1497.38) -- (181.29,1462.26) .. controls (190.99,1452.56) and (206.74,1452.59) .. (216.48,1462.32) .. controls (226.21,1472.05) and (226.24,1487.81) .. (216.54,1497.5) -- (181.42,1532.63) .. controls (171.72,1542.32) and (155.97,1542.3) .. (146.23,1532.56) .. controls (136.5,1522.83) and (136.47,1507.08) .. (146.17,1497.38) .. controls (155.87,1487.68) and (171.62,1487.71) .. (181.36,1497.44) .. controls (191.09,1507.17) and (191.12,1522.93) .. (181.42,1532.63) ;
%Straight Lines [id:da547224955867192] 
\draw    (47,1550) -- (305,1550) ;
%Shape: Ellipse [id:dp13529881602217309] 
\draw   (73,1522) .. controls (73,1518.13) and (81.28,1515) .. (91.5,1515) .. controls (101.72,1515) and (110,1518.13) .. (110,1522) .. controls (110,1525.87) and (101.72,1529) .. (91.5,1529) .. controls (81.28,1529) and (73,1525.87) .. (73,1522) -- cycle ;
%Shape: Ellipse [id:dp2318769342132868] 
\draw   (228,1523) .. controls (228,1519.13) and (236.28,1516) .. (246.5,1516) .. controls (256.72,1516) and (265,1519.13) .. (265,1523) .. controls (265,1526.87) and (256.72,1530) .. (246.5,1530) .. controls (236.28,1530) and (228,1526.87) .. (228,1523) -- cycle ;
%Shape: Circle [id:dp4630319343838194] 
\draw  [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][fill={rgb, 255:red, 244; green, 149; blue, 49 }  ,fill opacity=1 ] (159.83,1428.33) .. controls (159.83,1414.53) and (171.03,1403.33) .. (184.83,1403.33) .. controls (198.64,1403.33) and (209.83,1414.53) .. (209.83,1428.33) .. controls (209.83,1442.14) and (198.64,1453.33) .. (184.83,1453.33) .. controls (171.03,1453.33) and (159.83,1442.14) .. (159.83,1428.33) -- cycle ;
%Rounded Rect [id:dp6759304207856719] 
\draw   (181.79,1382.27) .. controls (181.79,1381.64) and (182.3,1381.13) .. (182.93,1381.13) -- (186.33,1381.13) .. controls (186.96,1381.13) and (187.47,1381.64) .. (187.47,1382.27) -- (187.47,1400.4) .. controls (187.47,1401.02) and (186.96,1401.53) .. (186.33,1401.53) -- (182.93,1401.53) .. controls (182.3,1401.53) and (181.79,1401.02) .. (181.79,1400.4) -- cycle ;
%Rounded Rect [id:dp6109099842166213] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (176.53,1374.05) .. controls (176.53,1372.33) and (177.93,1370.93) .. (179.65,1370.93) -- (189.01,1370.93) .. controls (190.74,1370.93) and (192.13,1372.33) .. (192.13,1374.05) -- (192.13,1388.21) .. controls (192.13,1389.94) and (190.74,1391.33) .. (189.01,1391.33) -- (179.65,1391.33) .. controls (177.93,1391.33) and (176.53,1389.94) .. (176.53,1388.21) -- cycle ;
%Shape: Cube [id:dp5334924952640538] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (167.83,1332.54) -- (188.04,1312.33) -- (217.33,1312.33) -- (217.33,1358.13) -- (197.13,1378.33) -- (167.83,1378.33) -- cycle ; \draw   (217.33,1312.33) -- (197.13,1332.54) -- (167.83,1332.54) ; \draw   (197.13,1332.54) -- (197.13,1378.33) ;
%Shape: Cube [id:dp5869800861415257] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (174.63,1299.83) -- (182.13,1292.33) -- (210.83,1292.33) -- (210.83,1319.04) -- (203.34,1326.54) -- (174.63,1326.54) -- cycle ; \draw   (210.83,1292.33) -- (203.34,1299.83) -- (174.63,1299.83) ; \draw   (203.34,1299.83) -- (203.34,1326.54) ;
%Rounded Rect [id:dp5074062073544287] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (186.73,1326.23) .. controls (186.73,1325.74) and (187.14,1325.33) .. (187.63,1325.33) -- (193.83,1325.33) .. controls (194.33,1325.33) and (194.73,1325.74) .. (194.73,1326.23) -- (194.73,1328.93) .. controls (194.73,1329.43) and (194.33,1329.83) .. (193.83,1329.83) -- (187.63,1329.83) .. controls (187.14,1329.83) and (186.73,1329.43) .. (186.73,1328.93) -- cycle ;
%Rounded Rect [id:dp07107841113389834] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (175.73,1326.23) .. controls (175.73,1325.74) and (176.14,1325.33) .. (176.63,1325.33) -- (182.83,1325.33) .. controls (183.33,1325.33) and (183.73,1325.74) .. (183.73,1326.23) -- (183.73,1328.93) .. controls (183.73,1329.43) and (183.33,1329.83) .. (182.83,1329.83) -- (176.63,1329.83) .. controls (176.14,1329.83) and (175.73,1329.43) .. (175.73,1328.93) -- cycle ;
%Shape: Diagonal Stripe [id:dp8330812749036848] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (192.43,1400.73) -- (199.83,1408.13) -- (170.23,1408.13) -- (177.63,1400.73) -- cycle ;
%Curve Lines [id:da944117454074688] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][line width=2.25]  [dash pattern={on 2.53pt off 3.02pt}]  (91.5,1515) .. controls (89.67,1489.68) and (110.63,1436.19) .. (175.91,1432.65) ;
\draw [shift={(179.97,1432.5)}, rotate = 538.74] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (14.29,-6.86) -- (0,0) -- (14.29,6.86) -- cycle    ;

% Text Node
\draw (193.5,1480.5) node  [font=\large] [align=left] {Obstacle};
% Text Node
\draw (265,1350) node  [font=\normalsize] [align=left] {\begin{minipage}[lt]{67.852644pt}\setlength\topsep{0pt}
\begin{center}
{\large Manipulator}\\{\large end-effector}
\end{center}

\end{minipage}};
% Text Node
\draw (88,1538.5) node  [font=\large] [align=left] {Initial point};
% Text Node
\draw (247,1538.5) node  [font=\large] [align=left] {Goal};


\end{tikzpicture}


==> figures/section_4/DDPG_base_architecture.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,2715); %set diagram left start at 0, and has height of 2715

%Straight Lines [id:da6348833137350979] 
\draw    (130,1191) -- (130,1251) ;


%Straight Lines [id:da8955672229771148] 
\draw    (220,1191) -- (220,1251) ;


%Straight Lines [id:da008980313535651097] 
\draw    (130,1211) -- (320,1211) ;


%Straight Lines [id:da7450816312462488] 
\draw    (130,1231) -- (320,1231) ;


%Straight Lines [id:da8976271619470423] 
\draw    (130,1270) -- (130,1330) ;


%Straight Lines [id:da41464090574227264] 
\draw    (220,1270) -- (220,1330) ;


%Straight Lines [id:da9112009599081309] 
\draw    (130,1290) -- (320,1290) ;


%Straight Lines [id:da5381713459343862] 
\draw    (130,1310) -- (320,1310) ;


%Straight Lines [id:da027284816905394194] 
\draw    (130,1351) -- (130,1411) ;


%Straight Lines [id:da16142919420184265] 
\draw    (220,1351) -- (220,1411) ;


%Straight Lines [id:da7828982960097542] 
\draw    (130,1371) -- (320,1371) ;


%Straight Lines [id:da8178584728252046] 
\draw    (130,1391) -- (320,1391) ;


%Straight Lines [id:da9968332046369773] 
\draw    (190,1250) -- (190,1267) ;
\draw [shift={(190,1270)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

%Rounded Rect [id:dp05506123650351347] 
\draw   (60,1197.29) .. controls (60,1193.26) and (63.26,1190) .. (67.29,1190) -- (312.71,1190) .. controls (316.74,1190) and (320,1193.26) .. (320,1197.29) -- (320,1242.71) .. controls (320,1246.74) and (316.74,1250) .. (312.71,1250) -- (67.29,1250) .. controls (63.26,1250) and (60,1246.74) .. (60,1242.71) -- cycle ;
%Rounded Rect [id:dp24412589443324362] 
\draw   (160,1078.5) .. controls (160,1073.81) and (163.81,1070) .. (168.5,1070) -- (521.5,1070) .. controls (526.19,1070) and (530,1073.81) .. (530,1078.5) -- (530,1131.5) .. controls (530,1136.19) and (526.19,1140) .. (521.5,1140) -- (168.5,1140) .. controls (163.81,1140) and (160,1136.19) .. (160,1131.5) -- cycle ;

%Straight Lines [id:da6150617955557683] 
\draw    (190,1140) -- (190,1187) ;
\draw [shift={(190,1190)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

%Rounded Rect [id:dp7093767239152369] 
\draw   (60,1277.29) .. controls (60,1273.26) and (63.26,1270) .. (67.29,1270) -- (312.71,1270) .. controls (316.74,1270) and (320,1273.26) .. (320,1277.29) -- (320,1322.71) .. controls (320,1326.74) and (316.74,1330) .. (312.71,1330) -- (67.29,1330) .. controls (63.26,1330) and (60,1326.74) .. (60,1322.71) -- cycle ;
%Straight Lines [id:da42531399150495086] 
\draw    (190,1330) -- (190,1348) ;
\draw [shift={(190,1351)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

%Rounded Rect [id:dp46046120438781557] 
\draw   (60,1358.29) .. controls (60,1354.26) and (63.26,1351) .. (67.29,1351) -- (312.71,1351) .. controls (316.74,1351) and (320,1354.26) .. (320,1358.29) -- (320,1403.71) .. controls (320,1407.74) and (316.74,1411) .. (312.71,1411) -- (67.29,1411) .. controls (63.26,1411) and (60,1407.74) .. (60,1403.71) -- cycle ;
%Rounded Rect [id:dp6858341803688754] 
\draw   (120,1587.29) .. controls (120,1583.26) and (123.26,1580) .. (127.29,1580) -- (252.71,1580) .. controls (256.74,1580) and (260,1583.26) .. (260,1587.29) -- (260,1632.71) .. controls (260,1636.74) and (256.74,1640) .. (252.71,1640) -- (127.29,1640) .. controls (123.26,1640) and (120,1636.74) .. (120,1632.71) -- cycle ;
%Straight Lines [id:da5593639963208532] 
\draw    (190,1410) -- (190,1577) ;
\draw [shift={(190,1580)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

%Rounded Rect [id:dp29114331445694763] 
\draw  [dash pattern={on 4.5pt off 4.5pt}] (51.5,1179) .. controls (51.5,1168.51) and (60.01,1160) .. (70.5,1160) -- (311,1160) .. controls (321.49,1160) and (330,1168.51) .. (330,1179) -- (330,1421) .. controls (330,1431.49) and (321.49,1440) .. (311,1440) -- (70.5,1440) .. controls (60.01,1440) and (51.5,1431.49) .. (51.5,1421) -- cycle ;
%Straight Lines [id:da4043771672351153] 
\draw    (430,1351) -- (430,1411) ;


%Straight Lines [id:da7008593578330864] 
\draw    (520,1351) -- (520,1411) ;


%Straight Lines [id:da2258584800837018] 
\draw    (430,1371) -- (620,1371) ;


%Straight Lines [id:da0323814069775088] 
\draw    (430,1391) -- (620,1391) ;


%Straight Lines [id:da5383953148115604] 
\draw    (431.5,1440) -- (431.5,1500) ;


%Straight Lines [id:da7008380759831091] 
\draw    (521.5,1440) -- (521.5,1500) ;


%Straight Lines [id:da9019044934568016] 
\draw    (431.5,1460) -- (621.5,1460) ;


%Straight Lines [id:da050021474746540395] 
\draw    (431.5,1480) -- (621.5,1480) ;


%Straight Lines [id:da8939502215813326] 
\draw    (431.5,1519) -- (431.5,1579) ;


%Straight Lines [id:da1710796465074278] 
\draw    (521.5,1519) -- (521.5,1579) ;


%Straight Lines [id:da2643574500611121] 
\draw    (431.5,1539) -- (621.5,1539) ;


%Straight Lines [id:da9843604516597262] 
\draw    (431.5,1559) -- (621.5,1559) ;


%Straight Lines [id:da7409263044210384] 
\draw    (500,1410) -- (500,1437) ;
\draw [shift={(500,1440)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

%Rounded Rect [id:dp8126523021173673] 
\draw   (360,1357.29) .. controls (360,1353.26) and (363.26,1350) .. (367.29,1350) -- (612.71,1350) .. controls (616.74,1350) and (620,1353.26) .. (620,1357.29) -- (620,1402.71) .. controls (620,1406.74) and (616.74,1410) .. (612.71,1410) -- (367.29,1410) .. controls (363.26,1410) and (360,1406.74) .. (360,1402.71) -- cycle ;
%Rounded Rect [id:dp6289788925360384] 
\draw   (361.5,1447.29) .. controls (361.5,1443.26) and (364.76,1440) .. (368.79,1440) -- (614.21,1440) .. controls (618.24,1440) and (621.5,1443.26) .. (621.5,1447.29) -- (621.5,1492.71) .. controls (621.5,1496.74) and (618.24,1500) .. (614.21,1500) -- (368.79,1500) .. controls (364.76,1500) and (361.5,1496.74) .. (361.5,1492.71) -- cycle ;
%Straight Lines [id:da96870266591465] 
\draw    (490,1500) -- (490,1516) ;
\draw [shift={(490,1519)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

%Rounded Rect [id:dp9249828069500274] 
\draw   (361.5,1526.29) .. controls (361.5,1522.26) and (364.76,1519) .. (368.79,1519) -- (614.21,1519) .. controls (618.24,1519) and (621.5,1522.26) .. (621.5,1526.29) -- (621.5,1571.71) .. controls (621.5,1575.74) and (618.24,1579) .. (614.21,1579) -- (368.79,1579) .. controls (364.76,1579) and (361.5,1575.74) .. (361.5,1571.71) -- cycle ;
%Rounded Rect [id:dp9354371841372842] 
\draw  [dash pattern={on 4.5pt off 4.5pt}] (351.5,1339.39) .. controls (351.5,1328.68) and (360.18,1320) .. (370.89,1320) -- (610.61,1320) .. controls (621.32,1320) and (630,1328.68) .. (630,1339.39) -- (630,1570.61) .. controls (630,1581.32) and (621.32,1590) .. (610.61,1590) -- (370.89,1590) .. controls (360.18,1590) and (351.5,1581.32) .. (351.5,1570.61) -- cycle ;
%Rounded Rect [id:dp8174445257453601] 
\draw   (470,1613.64) .. controls (470,1611.63) and (471.63,1610) .. (473.64,1610) -- (506.36,1610) .. controls (508.37,1610) and (510,1611.63) .. (510,1613.64) -- (510,1636.36) .. controls (510,1638.37) and (508.37,1640) .. (506.36,1640) -- (473.64,1640) .. controls (471.63,1640) and (470,1638.37) .. (470,1636.36) -- cycle ;
%Straight Lines [id:da7934941862447594] 
\draw    (490,1580) -- (490,1607) ;
\draw [shift={(490,1610)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

%Straight Lines [id:da36318237267719267] 
\draw    (190,1420) -- (460,1420) -- (460,1437) ;
\draw [shift={(460,1440)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

%Straight Lines [id:da8429981786555698] 
\draw    (490,1140) -- (490,1347) ;
\draw [shift={(490,1350)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;


% Text Node
\draw (190,1610) node [font=\Large] [align=center] {Action\\
$
[ f_{\mathrm{T} x} ,\ f_{\mathrm{T} y} ,\ f_{\mathrm{T} z}]
$};
% Text Node
\draw (571,1547.5) node   [align=left] {Linear};
% Text Node
\draw (268.5,1362.5) node   [align=left] {(None, 300)};
% Text Node
\draw (268.5,1399.5) node   [align=left] {(None, 3)};
% Text Node
\draw (93.5,1381.5) node   [align=left] {Dense};
% Text Node
\draw (175.5,1381.5) node   [align=left] {Activation};
% Text Node
\draw (165.5,1400.5) node   [align=left] {Output};
% Text Node
\draw (161.5,1361.5) node   [align=left] {Input};
% Text Node
\draw (269.5,1220.5) node   [align=left] {ReLU};
% Text Node
\draw (270,1278.5) node   [align=left] {(None, 400)};
% Text Node
\draw (268.5,1318.5) node   [align=left] {(None, 300)};
% Text Node
\draw (93.5,1300.5) node   [align=left] {Dense};
% Text Node
\draw (175.5,1298.5) node   [align=left] {Activation};
% Text Node
\draw (174,1318.5) node   [align=left] {Output};
% Text Node
\draw (172.5,1279.5) node   [align=left] {Input};
% Text Node
\draw (266,1380.5) node   [align=left] {tanh};
% Text Node
\draw (268.5,1238.5) node   [align=left] {(None, 400)};
% Text Node
\draw (266.5,1198.5) node   [align=left] {(None, 7)};
% Text Node
\draw (93.5,1221.5) node   [align=left] {Dense};
% Text Node
\draw (175.5,1221.5) node   [align=left] {Activation};
% Text Node
\draw (174,1240.5) node   [align=left] {Output};
% Text Node
\draw (172.5,1200.5) node   [align=left] {Input};
% Text Node
\draw (270.5,1299.5) node   [align=left] {ReLU};
% Text Node
\draw (248.5,1179.5) node   [align=left] {\textit{ACTOR}};
% Text Node
\draw (570,1530.5) node   [align=left] {(None, 300)};
% Text Node
\draw (572,1567.5) node   [align=left] {(None, 1)};
% Text Node
\draw (395,1549.5) node   [align=left] {Dense};
% Text Node
\draw (477,1549.5) node   [align=left] {Activation};
% Text Node
\draw (467,1568.5) node   [align=left] {Output};
% Text Node
\draw (463,1529.5) node   [align=left] {Input};
% Text Node
\draw (569.5,1380.5) node   [align=left] {ReLU};
% Text Node
\draw (571.5,1448.5) node   [align=left] {(None, 403)};
% Text Node
\draw (570,1488.5) node   [align=left] {(None, 300)};
% Text Node
\draw (395,1470.5) node   [align=left] {Dense};
% Text Node
\draw (477,1468.5) node   [align=left] {Activation};
% Text Node
\draw (475.5,1488.5) node   [align=left] {Output};
% Text Node
\draw (474,1449.5) node   [align=left] {Input};
% Text Node
\draw (568.5,1398.5) node   [align=left] {(None, 400)};
% Text Node
\draw (566.5,1358.5) node   [align=left] {(None, 7)};
% Text Node
\draw (393.5,1381.5) node   [align=left] {Dense};
% Text Node
\draw (475.5,1381.5) node   [align=left] {Activation};
% Text Node
\draw (474,1400.5) node   [align=left] {Output};
% Text Node
\draw (472.5,1360.5) node   [align=left] {Input};
% Text Node
\draw (572,1469.5) node   [align=left] {ReLU};
% Text Node
\draw (548.5,1339.5) node   [align=left] {\textit{CRITIC}};
% Text Node
\draw (490,1625) node    {$Q$};
% Text Node
\draw (345,1105) node [font=\Large] [align=center] {States\\
$
\left[\tilde{x}_{\mathrm{D}} ,\ \tilde{y}_{\mathrm{D}} ,\ \tilde{z}_{\mathrm{D}} ,\ \tilde{x}_{\mathrm{T}} ,\ \tilde{y}_{\mathrm{T}} ,\ \tilde{z}_{\mathrm{T}} ,\ \mathit{task}\right]
$};


\end{tikzpicture}


==> figures/section_4/axisDisplacement.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,5266); %set diagram left start at 0, and has height of 5266

%Shape: Axis 2D [id:dp8401731062472916] 
\draw [line width=1.5]  (57.09,103.02) -- (124.29,103.02)(57.09,44.77) -- (57.09,103.02) -- cycle (117.29,98.02) -- (124.29,103.02) -- (117.29,108.02) (52.09,51.77) -- (57.09,44.77) -- (62.09,51.77)  ;
%Straight Lines [id:da25787688788505003] 
\draw [line width=1.5]    (57.09,103.02) -- (24.08,132.08) ;
\draw [shift={(21.83,134.07)}, rotate = 318.63] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;

%Shape: Axis 2D [id:dp00030138802372781104] 
\draw [line width=1.5]  (166.3,160.92) -- (166.3,104.9)(96.43,160.92) -- (166.3,160.92) -- cycle (161.3,111.9) -- (166.3,104.9) -- (171.3,111.9) (103.43,165.92) -- (96.43,160.92) -- (103.43,155.92)  ;
%Straight Lines [id:da16248883132017578] 
\draw [line width=1.5]    (166.3,160.92) -- (130.04,194.34) ;
\draw [shift={(127.83,196.37)}, rotate = 317.33000000000004] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=1.5]    (14.21,-4.28) .. controls (9.04,-1.82) and (4.3,-0.39) .. (0,0) .. controls (4.3,0.39) and (9.04,1.82) .. (14.21,4.28)   ;

%Straight Lines [id:da6308765995432356] 
\draw [line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (57.09,103.02) -- (58.32,256.42) ;
%Straight Lines [id:da11858674863022223] 
\draw [line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (127.83,196.37) -- (58.32,256.42) ;


% Text Node
\draw (119,86) node    {$x_{T}$};
% Text Node
\draw (20,139) node    {$z_{T}$};
% Text Node
\draw (58,32) node    {$y_{T}$};
% Text Node
\draw (102,146) node    {$x_{D}$};
% Text Node
\draw (140,199) node    {$y_{D}$};
% Text Node
\draw (169,95) node    {$z_{D}$};
% Text Node
\draw (43,177) node  [rotate=-270]  {$0.07[\mathrm{m}]$};
% Text Node
\draw (99,199) node  [rotate=-317.3]  {$0.176\ [\mathrm{m}]$};
% Text Node
\draw (359,129.5) node    {$ \begin{array}{l}
XYZ\ =\ "0\ [\mathrm{m}] ,\ -0.07[\mathrm{m}] ,\ -0.176\ [\mathrm{m}] "\\
rpy\ =\ "0\ \mathrm{rad} ,\ 3.14\ \mathrm{rad} ,\ -1.57\ \mathrm{rad} "
\end{array}$};


\end{tikzpicture}


==> tables/section_5/simulation_testing_comparison.tex <==
\begin{tabular}{ccc}
	\hline 
	& \textbf{Mean} & \textbf{Std. Error}\\
	\hline 
	\textbf{Rewards}   & $-73.607$ & $8.608$ \\
	\textbf{Steps}   & $147.7$ & $4.676$\\
	\hline
\end{tabular}

==> tables/section_6/before_training.tex <==
\begin{tabular}{cccc}
    \hline
    \multicolumn{4}{c}{\textbf{Number of steps per epoch}}\\
    \hline
    & \textbf{Mean} & \textbf{Std. dev} & \textbf{Assistance}\\
    \hline
     \textbf{Subject 0} & & & \\
    \hline
    \multirow{2}{*}{\textbf{After training}} & $230.25$ & $63.86$ & - \\
    & $\mathbf{200.75}$ & $\mathbf{19.397}$ & \checkmark \\
    \hline
    \textbf{Subject 1} & & & \\
    \hline
    \multirow{2}{*}{\textbf{Before training}} & $496.25$ & $107.8$ & - \\
    & $\mathbf{487.5}$ & $\mathbf{54.51}$ & \checkmark\footnotemark \\
    \hline
    \multirow{2}{*}{\textbf{After training}} & $337.25$ & $79.65$ & - \\
    & $\mathbf{315.5}$ & $\mathbf{23.01}$ & \checkmark \\
    \hline
    \textbf{Subject 2} & & & \\
    \hline
    \multirow{2}{*}{\textbf{Before training}} & $300.25$ & $79.65$ & - \\
    & $\mathbf{275.0}$ & $\mathbf{55.76}$ & \checkmark\footnotemark[\value{footnote}] \\
    \hline
    \multirow{2}{*}{\textbf{After training}} & $208.5$ & $39.04$ & - \\
    & $\mathbf{166.25}$ & $\mathbf{44.31}$ & \checkmark \\
    \hline
\end{tabular}


% \begin{tabular}{ccccccc}
% 	\hline 
% 	&	\multicolumn{6}{c}{\textbf{Steps per episode before training}}\\
% 	\hline
% 		&\multicolumn{2}{c}{\textbf{Subject 0}}&\multicolumn{2}{c}{\textbf{Subject 1}}&\multicolumn{2}{c}{\textbf{Subject 2}}\\
% 		& \textbf{Mean} & \textbf{Std dev} & \textbf{Mean} & \textbf{Std dev} & \textbf{Mean} & \textbf{Std dev}\\
% 	\hline 
% 	\textbf{Without assistance}   & $-$ & $-$  & $496.25$ & $107.8$ & $300.25$ & $79.65$\\
% 	\textbf{With assistance}   & $-$ & $-$ & $487.5$ & $54.51$ & $275.0$ & $55.76$\\
% 	\hline
% \end{tabular}

% \begin{tabular}{ccccccc}
% 	\hline 
% 	&	\multicolumn{6}{c}{\textbf{Steps per episode after training}}\\
% 	\hline
% 		&\multicolumn{2}{c}{\textbf{Subject 0}}&\multicolumn{2}{c}{\textbf{Subject 1}}&\multicolumn{2}{c}{\textbf{Subject 2}}\\
% 		& \textbf{Mean} & \textbf{Std dev} & \textbf{Mean} & \textbf{Std dev} & \textbf{Mean} & \textbf{Std dev}\\
% 	\hline 
% 	\textbf{Without assistance}   & $230.25$ & $63.86$  & $337.25$ & $79.65$ & $208.5$ & $39.04$\\
% 	\textbf{With assistance}   & $200.75$ & $19.397$ & $315.5$ & $23.01$ & $166.25$ & $44.31$\\
% 	\hline
% \end{tabular}

==> tables/section_6/ddpg_second_comparison.tex <==
\begin{tabular}{c c}
	\hline 
% 	\multicolumn{4}{c}{SSTD Results}\\
	\textbf{Rewards}&\textbf{Steps}\\
	\hline 
	$-138.439$ & $145.5$\\
	\hline
\end{tabular}

%	\textbf{MTS}   & $-85.431$ & $160.5$\\
%	\textbf{STD}   & $-37.129$ & $94.3$\\
%	\textbf{E2E}   & $-37.758$ & $102.9$\\
%	\textbf{SSTD}   & $-36.729$ & $138$\\
%	\hline
%	\textbf{Normalized STD}   & $-66.302$ & $168.4$\\
%	\textbf{Normalized E2E}   & $-67.425$ & $183.75$\\
%	\hline

==> tables/section_6/forcesBefore.tex <==
\begin{tabular}{cccc}
    \hline
    \multicolumn{4}{c}{\textbf{Forces [N]}}\\
    \hline
    & \textbf{Max} & \textbf{Mean} & \textbf{Direction}\\
    \hline
    \textbf{Subject 0} & & & \\
    \hline
    \multirow{2}{*}{\textbf{After training}} & $1.549$ & $1.134$ & \textbf{Left} \\
    & $\mathbf{1.086}$ & $\mathbf{0.825}$ & \textbf{Right} \\
    \hline
    \textbf{Subject 1} & & & \\
    \hline
    \multirow{2}{*}{\textbf{Before training}} & $\mathbf{1.374}$ & $\mathbf{0.842}$ & \textbf{Left} \\
    & $0.992$ & $0.839$ & \textbf{Right} \\
    \hline
    \multirow{2}{*}{\textbf{After training}} & $1.12$ & $0.599$ & \textbf{Left} \\
    & $\mathbf{1.248}$ & $\mathbf{0.46}$ & \textbf{Right} \\
    \hline
    \textbf{Subject 2} & & & \\
    \hline
    \multirow{2}{*}{\textbf{Before training}} & $\mathbf{1.44}$ & $\mathbf{0.902}$ & \textbf{Left} \\
    & $1.418$ & $0.848$ & \textbf{Right} \\
    \hline
    \multirow{2}{*}{\textbf{After training}} & $1.52$ & $1.262$ & \textbf{Left} \\
    & $\mathbf{1.728}$ & $\mathbf{0.864}$ & \textbf{Right} \\
    \hline
\end{tabular}

% \
% \begin{tabular}{ccccccc}
% & \textbf{Mean}\\
%     \hline 
%     \textbf{Subject 0}   & $-$ & $-$ & $-$ & $-$ & $-$ & $-$\\
%     \textbf{Subject 1}   & $1.374$ & $0.535$ & $0.842$ & $0.992$ & $0.518$ & $0.839$\\
%     \textbf{Subject 2}   & $1.44$ & $0.134$ & $0.902$ & $1.418$ & $0.286$ & $0.848$\\
%  \hline
% \end{tabular}

% \begin{tabular}{ccccccc}
% & \textbf{Mean}\\
%     \hline 
%     \textbf{Subject 0}   & $1.549$ & $0.616$ & $1.134$ & $1.086$ & $0.575$ & $0.825$\\
%     \textbf{Subject 1}   & $1.12$ & $0.07$ & $0.599$ & $1.248$ & $0.197$ & $0.46$\\
%     \textbf{Subject 2}   & $1.52$ & $1.027$ & $1.262$ & $1.728$ & $0.212$ & $0.864$\\
%  \hline
% \end{tabular}

==> tables/section_6/velocityBefore_without_assistance.tex <==
\begin{tabular}{ccccc}
    \hline
    \multicolumn{5}{c}{\textbf{Velocity [cm/s]}}\\
    \hline
    & \textbf{Max} & \textbf{Mean} & \textbf{Direction} & \textbf{Assistance} \\
    \hline
    \textbf{Subject 0} & & & & \\
    \hline
    \multirow{4}{*}{\textbf{After training}} & $14.073$ & $6.229$ & \multirow{2}{*}{\textbf{Left}} & - \\
    & $\mathbf{22.38}$ & $\mathbf{8.988}$ & & \checkmark\\
    \cline{2-5}
    & $14.274$ & $5.949$ & \multirow{2}{*}{\textbf{Right}} & -\\
    & $\mathbf{17.688}$ & $\mathbf{6.73}$ & & \checkmark\\
    \hline
    \textbf{Subject 1} & & & & \\
    \hline
    \multirow{4}{*}{\textbf{Before training}} & $8.02$ & $3.166$ & \multirow{2}{*}{\textbf{Left}} & - \\
    & $\mathbf{10.987}$ & $\mathbf{3.779}$ & & \checkmark\footnotemark\\
    \cline{2-5}
    & $\mathbf{9.346}$ & $\mathbf{3.376}$ & \multirow{2}{*}{\textbf{Right}} & -\\
    & $8.973$ & $2.836$ & & \checkmark\footnotemark[\value{footnote}]\\
    \hline
    \multirow{4}{*}{\textbf{After training}} & $10.751$ & $4.861$ & \multirow{2}{*}{\textbf{Left}} & - \\
    & $\mathbf{11.328}$ & $\mathbf{4.848}$ & & \checkmark\\
    \cline{2-5}
    & $9.558$ & $4.076$ & \multirow{2}{*}{\textbf{Right}} & -\\
    & $\mathbf{13.175}$ & $\mathbf{4.578}$ & & \checkmark\\
    \hline
    \textbf{Subject 2} & & & & \\
    \hline
    \multirow{4}{*}{\textbf{Before training}} & $\mathbf{52.579}$ & $\mathbf{10.372}$ & \multirow{2}{*}{\textbf{Left}} & - \\
    & $44.915$ & $9.542$ & & \checkmark\footnotemark[\value{footnote}]\\
    \cline{2-5}
    & $27.692$ & $6.909$ & \multirow{2}{*}{\textbf{Right}} & -\\
    & $\mathbf{45.525}$ & $\mathbf{10.567}$ & & \checkmark\footnotemark[\value{footnote}]\\
    \hline
    \multirow{4}{*}{\textbf{After training}} & $14.849$ & $6.254$ & \multirow{2}{*}{\textbf{Left}} & - \\
    & $\mathbf{23.286}$ & $\mathbf{7.784}$ & & \checkmark\\
    \cline{2-5}
    & $23.75$ & $6.726$ & \multirow{2}{*}{\textbf{Right}} & -\\
    & $\mathbf{32.196}$ & $\mathbf{10.884}$ & & \checkmark\\
    \hline
\end{tabular}
